Digital Histopathology with Graph Neural Networks: Concepts and Explanations for Clinicians

To address the challenge of the ``black-box" nature of deep learning in medical settings, we combine GCExplainer - an automated concept discovery solution - along with Logic Explained Networks to provide global explanations for Graph Neural Networks. We demonstrate this using a generally applicable graph construction and classification pipeline, involving panoptic segmentation with HoVer-Net and cancer prediction with Graph Convolution Networks. By training on H&E slides of breast cancer, we show promising results in offering explainable and trustworthy AI tools for clinicians.

==> chapters/conclusion.tex <==
% Graph Signature
% Whole Slide Solutions
% HACT-NET
% Raman Spectrospecy as a different source
% Running CNN on optical density space instead of image space

% Effect of partially normalized vs smaller dataset effects vs no normalization.

% Human in the middle
    % Assists in stain normalization
    % Can help set parameters for watershedding etc.
    
\titlespacing{\section}{0pt}{1ex}{1ex}



\section{Results}
I am pleased to conclude that the requirements of my project were met, with all steps of the pipeline implemented. Due to the large scope of the project, the additional stipulation of performance at state of the art level was relaxed. This was not a shortcoming of the implementation, but rather the original proposal, which was based on unreasonable expectations. Regardless, I am pleased with the results, in particular with how my HoVer-Net implementation benchmarked against the original.

\section{Impact}
The impact of this project is two fold. Firstly, I demonstrate the continuing efficacy of graph based models for medical diagnosis. Although not pushing the state of the art forward, my model does demonstrate practical utility and with further fine-tuning I believe it would perform even better. Even though I make considerations pertinent to the diagnosis of breast cancer, the methodology was general and may be applied to cancers in others tissues, as well as different illnesses altogether.

Secondly, I applied a recent post-hoc explainability model (GCExplainer) to a new domain. I argued for an alternative graph representation algorithm, and proposed an additional metric for selecting the hyperparameter \textit{k}.

\section{Lessons Learned}
% Rewarding and challenging to work at the intersection of disciplines
It was both incredibly rewarding and challenging to work at the intersection of many disciplines. Programs with real world applications have the propensity for enormous impact, and, as motivated in the introduction, the fight against cancer is among the most important. Straying into the wild and away from the security of mathematical certainty, algorithms that operate over real world data are unlikely to work all the time, and I learned that imperfection in these situations should not be feared.

\section{Future Work}
% Neural and Symbolic approaches to explainability
The burgeoning field of AI explainability offers incredible value to the broader field of machine learning. It is to machine learning what the microscope was to biology; illuminating what was once unknown and opening doors to a new frontier of understanding. Reflecting back, the title of ``Towards Explainable AI for Cancer Diagnosis'' is incredibly fitting. This project is a step in the right direction, but more ambitious forms of explainability are required to overcome the final hurdle of machine learning adoption by doctors, and this demands further advancements in the field of XAI.

I believe a particular next-step worth pursuing is that of neurosymbolic models \cite{garcez2020neurosymbolic}. By reconciling traditional AI methods - such as first order logic and knowledge base systems - with deep learning approaches, there may be a capacity to process complex pieces of data while still reasoning about them logically. As a starting point, a project could explore applying Logic Explained Networks \cite{ciravegna2021logic} to GNNs.




==> chapters/evaluation.tex <==
\textit{In this chapter, I evaluate each stage of the project and give comparisons against existing implementations.}

\section{Challenges with Stain Normalization}
% POSSIBLY IMAGES OF SUCCESS
% How to evaluat
There are two main challenges that I faced normalizing real world examples:

 % Disambiguiating which is H&E 
 \begin{itemize}
     \item \textbf{A more informative third vector}: In some cases, where illumination is not uniform, the Macenko algorithm may pick up this lighting as one of the stain vectors, making the normalized image overly pink or purple in hue.
     
\begin{figure}[H]
    \centering
    \includegraphics[width=8cm,height=8cm,keepaspectratio]{Resources/failed_norm_1_v2.png} %

    \caption{Decomposition of original into stain saturation fails}%
    \label{fig:single_staining}%
\end{figure}

    \item \textbf{Stain vectors are too similar}: One of the steps in H\&E staining is the \textbf{differentiation} step where the stained sample is left in acid to selectively remove stains. A common problem is leaving the sample in too long (over-differentiating). As such, that particular stain will look faded, making it appear as though it were singularly stained; this is reflected in the similarity of the two discovered stain vectors.

\begin{figure}[H]
    \centering
    \subfloat[\centering]{{\includegraphics[width=6cm,height=4cm]{Resources/well_differentiated.png} }}%
    \qquad
    \subfloat[\centering]{{\includegraphics[width=6cm,height=4cm]{Resources/over_differentiated.png} }}%
    \caption{(a) Well differentiated vs (b) Over differentiated staining}%
    \label{fig:single_staining}%
\end{figure}

 \end{itemize}






%I developed a heuristic for determining if normalization would be ineffectual: see which target vectors the calculated stain vectors are closest to, and check that the two targets are different. From visual inspections, the heuristic does prevent normalizing to overly pink images, but is a little too conservative. Normalizing some images and not others partitions the dataset into two sets with very different stain statistics; This effectively makes a bi-modal dataset which may worsen predictive capabilities of later stages.

%\begin{figure}[H]
%    \centering
%    \includegraphics[width=14cm,height=2cm,keepaspectratio]{Resources/Ba%ch_stain_colours.PNG}
%    \caption{Top Two Rows: Extracted H\&E stains for BACH. Bottom Row: %Heuristic's decision to normalize (white = yes, black = no)}
%    \label{fig:bach_stain_vectors}
%\end{figure}



    %Problems with 2 from 3
 % Single Stained
    %Possibile degeneracies
 % My approach
 % Viz of all stain vector colours
 
 
\section{Nuclei Segmentation}
Since HoVerNet performs several tasks, I will quantitatively evaluate each one in turn.
\subsection{Instance Segmentation}
\label{sec:hover_inseg_eval}
There are two main facets to evaluating instance segmentation: how well are individual nuclei detected, and how precise are their segments. Because of its use in the graph construction, it is only the first of these responsibilities that we are interested in. Nonetheless, I evaluate both for completeness.

\subsubsection{Metrics}
Two popular evaluation metrics are the \textbf{Ensemble DICE} (DICE2) \cite{DICE2_paper} and \textbf{Aggregated Jaccard Index} (AJI) \cite{AJI_paper}. Both of these can be viewed as aggregations of simpler metrics:

\begin{align*}
 \text{DICE}(X,Y) & = \frac{2|X \cap Y|}{|X| + |Y|}\\
 \text{Jaccard Index}(X,Y)  & = \frac{|X \cap Y|}{|X \cup Y|}  
\end{align*}


In our case, X and Y would be the ground and predicted segment masks for a particular nuclei. Before aggregating, the ground and predicted nuclei are suitably assigned to one another based on their \textbf{IoU} (Intersection over Union).

There are some drawbacks to these metrics, including over-penalisation of overlapping regions, and so I used the \textbf{Panoptic Quality} (PQ) \cite{pquality} metric as well:


$$\mathcal{PQ} = \underbrace{\frac{|TP|}{|TP| + \frac{1}{2}|FP| + \frac{1}{2}|FN|}}_{\text{Detection Quality} (\mathcal{DQ})} \times 
\underbrace{\frac{\sum_{(x,y)\in TP}IoU(x,y)}{|TP|}}_{\text{Segmentation Quality} (\mathcal{SQ})}$$

The set of True Positive (TP) is obtained by optimally matching each ground segment to predicted segment; this was achieved by running the \textbf{Munkres assignment algorithm} \cite{kuhn1955hungarian} with a cost matrix storing pairwise IoU scores. The set of False Positives (FP) and Negatives (FN) are then acquired by taking the predicted and ground segments that were not matched. 

The \textbf{Detection Quality}(DQ) measures how well individual nuclei have been detected and the \textbf{Segmentation Quality}(SQ) measures how close each predicted segment is to the original.

\subsubsection{Results}
My trained implementation of HoVer-Net was evaluated on the \textbf{MoNuSeg} \cite{kumar2019multi} benchmarking dataset: 

\begin{table}[H]
\centering
\begin{tabular}{c|ccccc}
\textbf{Methods}                       & \textbf{PQ}   & \textbf{SQ}   & \textbf{DQ}    & \textbf{AJI}   & \textbf{DICE}   \\ \hline
\textbf{Cell Profiler} \cite{carpenter2006cellprofiler} & 0.300 & 0.704 & 0.423 & 0.366 & 0.623 \\
\textbf{QuPath} \cite{bankhead2017qupath}       & 0.351 & 0.679 & 0.511 & 0.432 & 0.696 \\
\textbf{FCN8} \cite{long2014fully}          & 0.312 & 0.714 & 0.434 & 0.281 & 0.797 \\
\textbf{FCN8 + WS} \cite{long2014fully}  & 0.425 & 0.719 & 0.590 & 0.429 & 0.797 \\
\textbf{SegNet} \cite{badrinarayanan2015segnet}       & 0.407 & 0.742 & 0.545 & 0.377 & 0.811 \\
\textbf{SegNet + WS} \cite{badrinarayanan2015segnet}  & 0.506 & 0.744 & 0.677 & 0.508 & 0.811 \\
\textbf{U-Net}  \cite{ronneberger2015u}      & 0.478 & 0.690 & 0.691 & 0.556 & 0.758 \\
\textbf{Mask-RCNN} \cite{he2017mask}   & 0.509 & 0.720 & 0.704 & 0.546 & 0.760 \\
\textbf{DCAN} \cite{chen2016dcan}         & 0.492 & 0.725 & 0.677 & 0.525 & 0.792 \\
\textbf{Micro-Net} \cite{raza2019micro}    & 0.519 & 0.747 & 0.692 & 0.560 & 0.797 \\
\textbf{DIST} \cite{naylor2018segmentation}       & 0.443 & 0.732 & 0.601 & 0.559 & 0.789 \\
\textbf{CIA-Net} \cite{zhou2019cia}       & 0.577 & 0.762 & 0.754 & 0.620 & 0.818 \\
\textbf{HoVer-Net} \cite{grahamHoVerNetSimultaneousSegmentation2019}    & 0.597 & \textbf{0.773} & 0.770 & 0.618 & \textbf{0.826} \\ \hline
\textbf{My Implementation} & \textbf{0.612}  & 0.691  & \textbf{0.887} & \textbf{0.624} & 0.774
\end{tabular}
\caption{Comparative results on the MoNuSeg dataset. WS denotes watershedding post processing.}
\label{tab:seg_results}
\end{table}

My results demonstrate capabilities around that of the original HoVer-Net implementation, producing a PQ score of \textbf{0.612} $\pm$ \textbf{0.021}. The model strikes a different trade-off in performance, favouring identification of nuclei over the quality of their segmentation. 

There are several hyperparameters used in the HoVer-Net post-processing, such as threshold values, and I observed the evaluation metrics were very sensitive to them. For example, a nucleus might be segmented in two because of a change in hyperparameters, causing a degradation of both SQ and DQ. To be consistent, I chose the same hyperparameters as those used in the HoVer-Net paper. 


\subsection{Classification}
\subsubsection{Metrics}
In the presence of unbalanced class sizes, solely using accuracy to evaluate classification is discouraged. Instead, it is suggested to use the following:

\begin{itemize}
    \item \textbf{Recall}: Measures how often a class is identified when an example is observed:
    $$R=\frac{TP}{TP+FN}$$
    \item \textbf{Precision}: When a class is predicted, how likely is it to be correct:
    $$P = \frac{TP}{TP + FP}$$
    \item \textbf{F1-Score}: Combines recall and precision:
    $$F1 = \frac{2(R\times P)}{R+P} = \frac{TP}{TP + \frac{1}{2}FN + \frac{1}{2}FP}$$
\end{itemize}

\subsubsection{Results}
The taxonomy of cell types used differs from dataset to dataset. Because of this incompatibility, I was only able to evaluate on a test partition of the PanNuke dataset:

\begin{table}[H]
\centering
\begin{tabular}{l|lll|lll|lll}
 & \multicolumn{3}{l|}{\textbf{Neoplastic}} & \multicolumn{3}{l|}{\textbf{Epithelial}} & \multicolumn{3}{l}{\textbf{Inflammatory}} \\ \cline{2-10} 
 & \textbf{R} & \textbf{P} & \textbf{F1} & \textbf{R} & \textbf{P} & \textbf{F1} & \textbf{R} & \textbf{P} & \textbf{F1} \\ \cline{2-10} 
\textbf{Micro-Net} \cite{raza2019micro} & 0.59 & 0.66 & 0.62 & \textbf{0.63} & 0.54 & \textbf{0.58} & 0.59 & 0.46 & 0.52 \\
\textbf{DIST} \cite{naylor2018segmentation} & 0.49 & 0.55 & 0.50 & 0.38 & 0.33 & 0.35 & 0.42 & 0.45 & 0.42 \\
\textbf{HoVer-Net} \cite{grahamHoVerNetSimultaneousSegmentation2019} & 0.58 & 0.67 & 0.62 & 0.54 & \textbf{0.60} & 0.56 & 0.56 & 0.51 & 0.54 \\ \hline
\textbf{My Implementation} & \textbf{0.69} & \textbf{0.70} & \textbf{0.69} & 0.55 & 0.47 & 0.51 & \textbf{0.69} & \textbf{0.58} & \textbf{0.63}
\end{tabular}
\end{table}

\begin{table}[H]
\centering
\begin{tabular}{l|lll|lll}
 & \multicolumn{3}{l|}{\textbf{Connective}} & \multicolumn{3}{l}{\textbf{Dead}} \\ \cline{2-7} 
 & \textbf{R} & \textbf{P} & \textbf{F1} & \textbf{R} & \textbf{P} & \textbf{F1} \\ \cline{2-7} 
\textbf{Micro-Net} \cite{raza2019micro} & 0.50 & 0.45 & 0.47 & 0.23 & 0.17 & 0.19 \\
\textbf{DIST} \cite{naylor2018segmentation} & 0.42 & 0.37 & 0.39 & 0 & 0 & 0 \\
\textbf{HoVer-Net} \cite{grahamHoVerNetSimultaneousSegmentation2019} & \textbf{0.52} & 0.47 & 0.49 & \textbf{0.28} & \textbf{0.35} & \textbf{0.31} \\ \hline
\textbf{My Implementation} & \textbf{0.52} & \textbf{0.62} & \textbf{0.57} & 0 & 0 & 0
\end{tabular}

\caption{Comparative results on the PanNuke dataset.}
\label{tab:hover_class}
\end{table}


\begin{figure}[H]
    \centering
    \includegraphics[width=14cm,height=8cm,keepaspectratio]{Resources/cf.PNG}
    \caption{Confusion matrix for cell types}
    \label{fig:confusion_matrix}
\end{figure}

% Mention of no examples of dead cells in Breast example in PanNuke


The results are again comparable with the original HoVer-Net metrics. A particular shortcoming with the trained model is its inability to detect dead cells. Because HoVer-Net is used for breast tissue downstream, this would only be a problem if there are a considerable number of dead cells in the tissue. However, this is not the case as can be seen in Figure \ref{fig:pannuke_dist}. There are virtually no dead cells in the breast tissue examples, featuring primarily in lung tissue instead.

Please note that the size of training, validation and test partitions differ from the benchmarks: I used and 80/0/20 split compared to a 33/33/33 split by the other authors.




 \section{Cancer Prediction}
 This evaluation will span both the choice of graph definitions as well as the performance of my GNN.
 
 \subsection{Over-Smoothing}
 \label{sec:eval_knn}
 Over-smoothing \cite{chen2020measuring} is a fundamental challenge for graph neural networks: nodes that receive an almost complete description of the entire network cannot provide new and interesting information for their neighbours to learn from.
 
 A KNN graph was chosen over a radius based graph\footnote{A graph where nodes are connected if they are within a certain radius of one another} because it gave fully connected cell-graphs without a quadratic number of edges. It is in a complete graph, where there are a quadratic number of edges, that over-smoothing is most likely to occur.

 
  \subsection{Results}
The GNN was trained and tested on cell graphs derived from the original BACH dataset. Some images contained few to no cells and had to be discarded, leaving 386/400 graphs; in these cases, no cancer was present as tumours cannot form without cells. I again take an 80/20 split, making sure to keep the proportions of each class balanced.

\begin{figure}[H]
    \centering
    \includegraphics[width=8cm,height=8cm,keepaspectratio]{Resources/confusion_matrix_gnn.PNG}
    \caption{Confusion matrix for cancer predictions}
    \label{fig:confusion_matrix_gnn}
\end{figure}


The four class test accuracy was \textbf{82\%}, and the two class (cancer or not cancer) test accuracy was \textbf{87\%}. In the original BACH grand challenge, the top score was \textbf{87\%} on a held out test set, with my model breaking into the top-10 assuming my test accuracy translates. I am satisfied with the four class test accuracy, but surprised with the marginal improvement for two classes. The model ideally would have learned that normal \& benign and in-situ \& invasive are similar to one another, and hence most of the uncertainty would be in differentiating within these pairs. \cite{deepakanandHistographsGraphsHistopathology2020} quote 93\% accuracy for two classes but used a network with over 1000x more parameters. \cite{wang2021cell}'s models reached an accuracy of 79 $\pm$ 3\% for gastric cancer with three classes. These comparisons point to my implementation being consistent with modern results for cancer diagnosis.

\begin{figure}[H]
    \centering
    \includegraphics[width=8cm,height=8cm,keepaspectratio]{Resources/training_plot_gnn.png}
    \caption{Training plot for the GNN, with loss against number of steps. A loss of 1.4 corresponds to random guessing. Training loss is taken across batches, while validation loss is taken across the entire epoch.}
    \label{fig:training_plot_gnn}
\end{figure}

Unfortunately, the plot is misleading. Validation loss did indeed reach 0.56 but epoch training loss was lower at 0.30; I believe this was an artifact of plotting batch loss for small batches. This suggests there was some overfitting, and with some more tuning, such as increasing dropout and weight decay, this may have been reduced further. 


  % Training plots
  % Results for BACH
  % Admissible performance, requires a lot more tuning which was not necessary for project
  % Suprising that canc accuracy is marginally better
 % WHY GCN OVER GIN AND TOPK
 
\section{Explainability}
 GCExplainer proposed two evaluations metrics. In this discussion, I explore each in turn and retrofit them as much as possible to this project. 


\subsection{Concept Completeness}
Concepts should be good indicators, and predictions based solely on concepts should be accurate. Taken to the extreme, how accurate is a classifier that predicts the most frequent class given a single concept? This is the concept completeness score, and it can be calculated by training and evaluating a decision tree.

There are two things I want to mention. Firstly, the score was low at 53\% accurate on a node by node basis, but if instead predictions are made using all nodes within a graph, an accuracy of 73\% was reached, closer to the power of the GNN. GCExplainer was primarily evaluated on synthetic datasets for which GNNs perform extremely well. It was observed that real-world datasets are much harder to explain than their synthetic counterparts. For perspective, completeness scores of 96\% and 95\% were achieved on the BA-Shapes \cite{ying2019gnnexplainer} and REDDIT-BINARY \cite{morris2020tudataset} datasets respectively.

Secondly, the concept completeness score can be used to select \textit{k}. Unfortunately, I did not observe a significant change in score as \textit{k} was varied, so I was forced to try alternative metrics. I defined a \textbf{minimum prevelance score} (MPS) as a proxy for how ``local'' concepts are. This is calculated by counting how many different samples a concept features in, and taking the smallest count as a percentage of the training set. I eventually chose 32 because this was the size of the network and the MPS was just starting to dip below 10\%.
\begin{figure}[H]
    \centering
    \includegraphics[width=12cm,height=8cm,keepaspectratio]{Resources/min_prev_score.PNG}
    \label{fig:min_prev_score}
    \caption{}
\end{figure}


\subsection{Concept Purity}
Concept purity measures how coherent concept representations are. The original motivation was that the top-3 concepts should roughly all contain the same nodes and edges. The graph edit distance \cite{riesen2015structural}, calculated through graph alignment, is a measure of graph dissimilarity and is taken to be the concept purity. 

I took concepts to be a group of clustered cells exhibiting some shared trait, as was reflected in my interpretation in \S \ref{sec:concept_interpretation}. It was for this reason that concepts should be represented by the subgraph of conceptually identical nodes, as opposed to the \textit{n}-hop neighbourhood, as it did not make sense to include nodes of a different concept within the representation. Because edges between nodes are too predictable in a KNN definition and all nodes within a representation are the same, the concept purity was not applicable. 

Although the representation of concepts was different, concept discovery and assignment remains unchanged. This is because concepts are calculated and assigned before the representation step, so are irrespective of it.

 


    


==> chapters/implementation.tex <==
\textit{In this chapter, I walk through each of the five pipeline steps of my project, expanding on implementation details and design decisions. I begin with an overview and a mentioning of the datasets used.}

\section{Overview of Pipeline}
The below diagram provides a richer definition of the project stages but stays true to Figure \ref{fig:coarse_overview}. 

\begin{figure}[H]
    \centering
    \includegraphics[height=15cm,keepaspectratio]{Resources/Full Overview.png}
    \caption{The five colours correspond to the five pipeline steps.}
    \label{fig:full_overview}
\end{figure}

\section{Datasets}
Even though the volume of digitized clinical data is large,  it is still difficult for small research groups to acquire large medical datasets. This is because: they are labor intensive to collate and annotate, the size of each datapoint can be very large, and privacy policies prevent them from becoming publicly available.

A successful remedy has been to compile datasets for competitions. These sets not only provide sufficient data to train, but also provide a standard for benchmarking. I will briefly describe the datasets I made use of:

\subsection{PanNuke}
The \textbf{PanNuke} dataset \cite{gamperPanNukeDatasetExtension2020} contains segmentation masks for nearly 200,000 labelled nuclei across 
over 7,000 images. Samples range across 19 different tissue types and 5 cell types: neoplastic, epithelial, inflammatory, connective and dead. It should be noted that breast tissue was the most common tissue sample in the set.

\begin{figure}[H]
    \centering
    \includegraphics[width=6cm,height=6cm,keepaspectratio]{Resources/pannuke_dist.PNG}
    \caption{Distribution of cell types in PanNuke}
    \label{fig:pannuke_dist}
\end{figure}



\subsection{BACH}
The \textbf{BreAst Cancer Histology images} (BACH) dataset consists of 400 H\&E images of breast tissue. Each image is in one of \textbf{four} classes (with each class containing 100 examples): \textbf{Normal}, \textbf{Benign}, \textbf{In-Situ}, and \textbf{Invasive}. The last two classes are cancerous, while the first two are not.







\section{Stain Normalisation}
\label{sec:stain_norm}
% SOMETHING ABOUT STAIN VECTORS being not the same
% TODO Define better task
The purple and pink hues of the Hematoxylin and Eosin stains may differ from image to image. To put it simply, stain normalisation makes all the pinks and purples the same across samples. Macenko et al.\cite{macenko2009method} present a method for performing this type of normalisation. Below, I explain their approach and how I specifically applied it to H\&E staining. 
    \subsection{Macenko Algorithm}

The principal goal of the Macenko algorithm is to decompose the pigmentation of each pixel into a linear combination of the stain vectors. Where pixels appear dark, the tissue is particularly stained and hence absorbs (or attenuates) the light passing through. The \textbf{absorbance} or \textbf{optical density} of a material can be calculated by $-log(\frac{I_t}{I_r})$ where $I_t$ and $I_r$ are the radiance transmitted and received by the material. In optical density space, linear combinations of stains leads to linear combinations of optical density values \cite{fawcett1960rapid}. By making the conversion of RGB intensities to optical density space: $$D = -log(I)$$our task reduces to decomposing $D$ into a matrix of \textbf{stain vectors} $V$ and their relative \textbf{saturations} $S$:$$D = VS$$

% IMAGE OF EACH PIXEL IN THE TWO SPACES

\begin{figure}[H]
    \centering
    \includegraphics[width=12cm,height=6cm,keepaspectratio]{Resources/Pixel Intensities in diff space.PNG}
    \caption{Pixel Intensities in the Different Spaces}
    \label{fig:pixel_intensity}
\end{figure}
% Intrinsiclly 2 channel data in 3 channel space. Use dimensionality reduction (i.e. PCA) to find 2 most informative axis, then project all points onto the plane.
Since there are two stain vectors in H\&E, $V$ defines a 2-dimensional subspace within the 3-dimensional optical density space, where the stain vectors are the basis. Principle Component Analysis (PCA), a form of dimensionality reduction, can be used to discover this subspace. PCA finds a smaller set of basis (2 instead of 3) such that the sum of squared distances of points to their projection on this subspace is minimized\footnote{This goal seeks for reconstructed points to be  as close as possible to their original, and thus preserves much of the information}. It can be shown \cite{Goodfellow-et-al-2016} that this space is equal to the space spanned by the most important\footnote{Eigenvectors with largest eigenvalues} eigenvectors of the covariance matrix, as well as the most important right singular vectors of the data matrix. Each point is then projected onto this space. Points in this space can be parameterised by two non-negative scalars, specifying the quantity of each stain vector. 

$$p(\lambda_1,\lambda_2) = \lambda_1\bar{v_h} + \lambda_2\bar{v_e}$$

This implies that all points lie within a triangular region, bound by the two stain vectors. We therefore have a recipe for determining $v_1$ and $v_2$: find direction parallel to region's border by comparing data points which make the smallest and largest angles with the principle components.

In practise, noise can artificially move points outside of the envelope. To make the approach more robust, low pigmented pixels are not considered (controlled by $\beta$~-~the minimum threshold) and vectors with less extreme angles are used instead (controlled by $\alpha$ - the angle percentile to use).

% Use alpha and beta hyperparameters to control noise.
\begin{figure}[H]
    \centering
    \includegraphics[width=8cm,height=6cm,keepaspectratio]{Resources/finding stain_vecs.PNG}
    \caption{Visualization of possible stain pairs, with different alphas, and beta=0.15}
    \label{fig:OD_inHE_space}
\end{figure}

\begin{algorithm}[H]
\caption{For Determining Stain Vectors in OD Space}\label{alg:stain_vect}
\begin{algorithmic}[1]
\State $D \gets -log(I)$ \Comment{Converts pixel intensities into OD space.}
\State Remove data with OD intensity below $\beta$.
\State $U,\Sigma,V^T \gets SVD(D)$
\State $b_1,b_2 \gets $ right singular vectors (from $V^T$) with largest singular values.
\State Project points onto plane, then normalize. \Comment{Makes it easier to find angle.}
\State Calculate angle of each point w.r.t second right singular vector.
\State Take $\alpha^{th}$ and $(100-\alpha)^{th}$ percentiles of angles as the min and max angles.
\State Stain Vector $\gets \begin{pmatrix}
  b_1 & b_2\end{pmatrix}\begin{pmatrix}
  cos(\theta)\\
  sin(\theta)
\end{pmatrix}$ for min and max angles.
\end{algorithmic}
\end{algorithm}

% Diagram of process

% TODO Stress that target will be same across the entire dataset
% After finding vectors, demonstrate deconvolution. Demonstrate change of vectors.
Once the stain vectors $V$ have been found for all images, we can normalise by multiplying the relative saturations by a common set of stain vectors $V_{norm}$:

$$D = VS \implies S = V^{-1}D$$
\begin{equation}
    D_{norm} = V_{norm}S = V_{norm}V^{-1}D
\end{equation}

\begin{figure}[H]
    \centering
    \includegraphics[width=14cm,height=5cm,keepaspectratio]{Resources/normalized images.PNG}
    \caption{Image Normalization Comparison}
    \label{fig:norm}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=14cm,height=5cm,keepaspectratio]{Resources/deconv.png}
    \caption{Deconvolution into Hematoxylin and Eosin stains }
    \label{fig:deconv}
\end{figure}


% TODO: Where this code can be found
 
 
\section{Nuclei Segmentation with HoVer-Net}
My cell graph schema requires that both instances and types of cells/nuclei are identified. Among the hardest challenges with instance segmentation of nuclei is separating neighbouring or overlapping nuclei; this problem is broadly referred to as \textbf{under-segmentation} where too few segments have been defined.

To accomplish this, I used a deep learning architecture called \textbf{HoVer-Net} \cite{grahamHoVerNetSimultaneousSegmentation2019}, in combination with classical post processing steps. Their approach was specifically designed to address the aforementioned challenge.

%TODO OUTLINE WHAT FCN means

\subsection{Architecture}
Like many other segmentation architectures, Horizontal Vertical Network or \textbf{HoVer-Net} is an encoder-decoder network, but unlike them, it uses multiple (three) decoding branches to achieve panoptic segmentation. I will explain what an encoder-decoder network is and then explain details pertinent to HoVer-Net.

The terms encoder and decoder originate from information theory where a signal is first encoded before entering the channel, after which it is decoded and recovered. Certain desirable properties, like noise resistance and storage efficiency, will be better utilized under certain representations, and the process of encoding and decoding corresponds to translations between such representations.

\label{sec:auto_encoders}
Neural encoders seek to find a meaningful and informative representation for their input. If this representation lives in a lower dimension, then this approach leads to a probabilistic compression algorithm. Such architectures are referred to as \textbf{autoencoders}. 

As well as learning the identity function, the encoder-decoder network can learn to translate inputs from one domain to another; in this case, the decoder does not map back to the original space. For example, Sequence-to-Sequence \cite{sutskever2014sequence} models perform literal translation from one language to another. In \S \ref{sec:decoder}, I show how suitable decoders can be used to translate pixels to classes and thus perform semantic segmentation.

\begin{figure}[H]
    \centering
    \includegraphics[width=14cm,height=8cm,keepaspectratio]{Resources/hovernet.jpg}
    \caption{HoVer-Net architecture, as presented in \cite{grahamHoVerNetSimultaneousSegmentation2019}. The residual units make up the encoder branch, which is followed by three near identical decoder branches}
    \label{fig:hovernet-arch}
\end{figure}


\subsubsection{Encoder}
% TODO SAY LOTS MORE ON ARCHITECTURE: what is a FCN, how is down sampling doone, what is the activation function, what is batchnorm.

The encoder is almost identical to ResNet-50, a certain specification of the ResNet architecture. It is defined by stacking so-called ``residual units'' which are blocks of layers with a skip connection. These blocks interleave convolutional layers between activation and normalisation layers. The activation layer used is the Rectified Linear Unit or \textbf{ReLu} where:
$$\sigma(x) = 
\begin{cases} 
    x \quad \text{if } x > 0 \\
    0 \quad \text{if } x \leq 0 
\end{cases}$$

Downsampling is performed with a stride of 2 on specific convolutional layers. The authors suggest using three downsamples instead of the four which ResNet-50 would otherwise suggest.
\subsubsection{Decoders}
\label{sec:decoder}
The output of the encoder is fed into three dedicated decoder branches.
These branches are identical in all but the head (the last layer) used. Below I describe their role:
%\footnote{This task was earlier accomplished by the U-Net\cite{ronneberger2015u} architecture}
\begin{itemize}
    \item \textbf{Nuclear Pixel (NP) branch}: This branch performs semantic binary segmentation to predict if a pixel is either part of a nucleus or not. The head consists of a convolutional layer followed by a sigmoid activation function.
    
    \item \textbf{HoVer branch}: This branch learns to find the displacement of pixels from their nucleus' centre of mass. The head of the decoder has two channels, one for learning horizontal displacements and one for vertical. These values range from -1 for far left/top to 1 for far right/bottom. The head is just a 2 channel convolutional layer\footnote{Though the output is unbound, placing an activation function like \textbf{tanh} to get outputs between -1 and 1 made the model perform worse.}. See figure \ref{fig:hover_map_example} for an example.
    
    \item \textbf{Nuclear Classification (NC) branch}: The role of the third branch is to predict the nucleus type via semantic segmentation. The head is made of a 6 channel convolutional layer followed by a softmax layer. The first five layers are for the five possible cell type, and the sixth is for the background.
    
    %The HoVer-Net paper explored the consequences of classifying cells using instead an additional head on the NP branch, but found that performance was inferior to using a dedicated branch. This is because the task of 

\end{itemize}
In Section \ref{sec:hvn_post}, I show how the outputs of the NP and HoVer branches can be used to perform instance segmentation, even in the presence of overlapping nuclei.










\subsection{Training}
I now skim over a variety of steps run before and during training, before spending time defining the network's loss function.

\textbf{Hyperparameter Injection:} for all trainers, I made hyperparameters injectible by using loading a JSON file. This allowed me to, for example, change the encoder complexity to any of the ResNet \cite{resnet} specifications by specifying a width, and to change the min and max learning rate.

\textbf{Data Preperation:} %todo: rewrite to be clearer
I trained HoVer-Net with the PanNuke dataset, which had ground truths for panoptic segmentation. It was only necessary for me to create labels for the second branch, namely ``hover maps".

\begin{figure}[H]
    \centering
    \subfloat[\centering]{{\includegraphics[width=4cm,height=4cm]{Resources/h_map_example.PNG} }}%
    \qquad
    \subfloat[\centering]{{\includegraphics[width=4cm,height=4cm]{Resources/v_map_example.PNG} }}%
    \caption{Horizontal (a) and Vertical (b) map examples}%
    \label{fig:hover_map_example}%
\end{figure}

\iffalse
\begin{algorithm}[H]
\caption{For generating hover maps}\label{alg:hover_maps}
\begin{algorithmic}[1]
\Require{$im$ (Instance Mask)} \Comment{Nuclei labelled 1 to N, background 0}

\State $H_{map},V_{map} \gets$ torch.zeros(height,width)
\State X,Y $\gets$ each pixel's x and y coordinates 
\For{nid in RANGE(1,N)}
    \State mask $\gets$ $im==nid$ \Comment{Mask for nucleus $nid$}
    \State $X_\mu,Y_\mu \gets (X*mask).mean,(Y*mask).mean$  \Comment{The coordinates of the nucleus centre of mass}
    \State $X_\delta,Y_\delta \gets (X-X_\mu)*mask,(Y-Y_\mu)*mask$ \Comment{Displacement of each pixel in nucleus boundary}
    \State $X_\delta,Y_\delta \gets norm(X_\delta),norm(Y_\delta)$ \Comment{Normalizes to -1 and 1, keeping 0 invariant}
    \State $H_{map},V_{map} += X_\delta,Y_\delta$ \Comment{Add the displacement for nucleus $nid$ to aggregate}
\EndFor
\end{algorithmic}
\end{algorithm}
\fi

%\textbf{Optimizer}

%TODO Elaborate!
\textbf{Data Augmentation:} I used a series of data augmentation techniques to artificially enlarge the dataset. I used standard operations like flip, crop, noise and blur, as well as the less common elastic deformer. In addition, I used a H\&E colour jitterer that perturbs the stain vectors of the image. As mentioned in section \ref{sec:gdl}, one can encode geometric priors through augmentations to the data, and the invariance under stain colours is one such prior I chose to encode.


%\textbf{Hyperparameter Injection}


\textbf{One Cycle Learning:} Proposed by \cite{one_cycle}, this learning rate curriculum has been used in practise to improve model performance. The learning rate smoothly goes from the starting rate, to a maximum, then down to 0, across the entire experiment. This approach can be compared to simulated annealing, and I used it in each model I trained throughout the project.

\subsubsection{Loss Function}
\label{sec:loss_hover}
We can associate a loss with each of the three branches / tasks. To get a loss function for the entire network, we can just take the weighted sum of these losses. I present this aggregate loss function below with the weights I used and then go on to explain each of the component losses:

$$\mathcal{L} = \underbrace{\mathcal{L}_a + 2\mathcal{L}_b}_\text{HoVer Branch}+ \underbrace{\mathcal{L}_c + \mathcal{L}_d}_\text{NP Branch} + \underbrace{\mathcal{L}_e + \mathcal{L}_f}_\text{NC Branch}$$



Since the HoVer branch is performing regression, it makes sense to use \textbf{mean squared error} (MSE). $\mathcal{L}_a$ is the MSE of the predicted ($\hat{h}$) to target hover maps ($h$). The model needs to understand that within cells the prediction should grow linearly as you move horizontally and vertically. Additionally, the model needs to appreciate the discontinuity at the borders of cells, and should be penalised for not adhering to it. These two requirements are captured in $\mathcal{L}_b$ in which the MSE is taken over the gradients of the predicted and target hover maps.
$$\mathcal{L}_a = \frac{1}{N}\sum_{d \in\{x,y\}}\sum_{i}^{N} ||h_d(i)-\hat{h}_d(i)||_2^2$$

$$\mathcal{L}_b = \frac{1}{N}\sum_{d \in\{x,y\}}\sum_{i}^{N} ||\nabla_d (h_d(i))-\nabla_d (\hat{h}_d(i))||_2^2$$

For the \textbf{NP} and \textbf{NC} branches, I use both cross entropy loss and dice loss. The cross entropy loss is a measure of the distance between two distributions. It is frequently used in classification and segmentation tasks because models usually output a degree of belief / probability distribution for each class.

$$CE = -\frac{1}{N}\sum^K_c\sum^N_i p(i,c) log(\hat{p}(i,c))$$

where i and c index pixels and classes respectively. The DICE coefficient is used to evaluate a segmentation prediction by seeing how well target and predicted segments overlap. For each class $c$, we can calculate this by computing:

$$\text{DICE Coefficient}_c = \frac{2 \sum_i p(i,c)\times \hat{p}(i,c)}{\sum_i p(i,c) + \sum_i \hat{p}(i,c)}$$

One can view multiplication in the numerator as the soft equivalent of taking an intersection, and the addition on the denominator as taking the disjoint union\footnote{See \ref{sec:hover_inseg_eval} for hard equivalent.}. A score of 1 corresponds to perfect overlap and 0 to no overlap at all. To turn this into a loss, we subtract from 1. Finally, we take a mean of all the component DICE losses to get the aggregate DICE loss.

$$DICE = \sum_c 1- \frac{2 \sum_i p(i,c)\times \hat{p}(i,c)}{\sum_i p(i,c) + \sum_i \hat{p}(i,c)}$$

$\mathcal{L}_c$ \& $\mathcal{L}_e$ are the cross-entropy losses for the \textbf{NP} and \textbf{NC} branches, and $\mathcal{L}_d$ \& $\mathcal{L}_f$ are their DICE losses. Note that K equals 2 \& 6 for the \textbf{NP} and \textbf{NC} branches respectively, and $p(i,c)$ \& $\hat{p}(i,c)$ are those branches' target and predicted outputs.
    
\subsection{Classical Postprocessing}
\label{sec:hvn_post} 
\subsubsection{Tiling}
The deep learning model contains over 50 million parameters. It requires 8GB of memory to pass a 256x256 image through the network. It is therefore necessary to chunk up a large image and then tile the predictions. 

\subsubsection{Watershedding}
\label{sec:watershedding}
In order to produce the instance segmentation mask, the outputs of the NP and Hover branches are processed with a series of classical computer vision algorithms. At the heart of this stage is the \textbf{watershedding} algorithm. Its name comes from topography where the term refers to the division of two drainage basins as a result of elevated land. Given an \textbf{energy landscape}\footnote{A 1 channel image that stores the relative height of a point on the ``map''} and \textbf{markers} for the basins, the algorithm will fill the cavities until the water spills into adjacent basins.

The way in which the landscape is defined and the markers selected are key factors in determining how well regions are segmented. I present the methodology used in the HoVerNet paper.

Firstly, a landscape is derived that places a ridge around cells. This is accomplished by applying Sobel filters to the predicted hover maps. There are two Sobel filters and they compute horizontal and vertical approximations to the gradients. Consider applying the horizontal Sobel filter to the horizontal hover map. The background will receive a value of 0 and the inside of the cells will recieve a positive value (as the displacement from the centre increases linearly). In addition, the left and right border will receive a large negative and positive value respectively because of the discontinuity. By taking the absolute value, the left and right edges effectively become ridges. This step is repeated for the vertical direction, and then I take the maximum across both directions to get edges in all directions.

\begin{equation}
    L = max(S_x(h_x),S_y(h_y))
\end{equation}
where $S_x$ \& $S_y$ are the horizontal and vertical Sobel filters and $h_x$ \& $h_y$ are the two hover maps.

\begin{figure}[H]
    \centering
    \subfloat[\centering]{{\includegraphics[width=10cm,height=4cm,keepaspectratio]{Resources/hover_net_example/original_example.PNG} }}%
    \qquad
    \subfloat[\centering]{{\includegraphics[width=10cm,height=4cm,keepaspectratio]{Resources/hover_net_example/h_map.PNG} }}%
    \qquad
    \subfloat[\centering]{{\includegraphics[width=4cm,height=4cm]{Resources/hover_net_example/sobelled.PNG} }}%
    \caption{Original (a), Predicted Horizontal Map (b), Energy Landscape L (c)}%
    \label{fig:hovernet_importance}%
\end{figure}

Next, a mask is generated to reconcile the landscape with the nuclear pixel prediction. I apply thresholding to the output of the \textbf{NP} branch with values above 0.5 going to 1 and the values below going to 0. This mask is then placed on top of the landscape so that edges which are false positives are removed; this is a byproduct of using multiple decoding branches as predictions may contradict each other, albeit with high uncertainty.


At this point, the landscape is such that depressions are within nuclei and elevations are along the borders. A single marker will be taken at each of these depressions from which the region will grow from. Again, the depressions can be calculated with thresholding, with each marker spanning a small area. 

At last, watershedding can be applied.

\begin{figure}[H]
    \centering
    \subfloat[\centering]{{\includegraphics[width=10cm,height=4cm,keepaspectratio]{Resources/hover_net_example/np_prediction.PNG} }}%
    \qquad
    \subfloat[\centering]{{\includegraphics[width=10cm,height=4cm,keepaspectratio]{Resources/hover_net_example/markers.PNG} }}%
    \qquad
    \subfloat[\centering]{{\includegraphics[width=10cm,height=4cm,keepaspectratio]{Resources/hover_net_example/instance_masks.PNG} }}%
    \caption{Predicted Semantic Mask (NP output) (a), Markers (b), Predicted Instance Mask (c)}%
    \label{fig:hovernet_instance_seg}%
\end{figure}

\subsubsection{Nucleus Type Prediction}
\label{sec:nucleus_type}
The very last step is to assign a prediction to each nucleus. This is achieved by applying the nuclear mask to the output of the \textbf{NC} branch, and then taking a \textbf{majority vote} across all classes (except background).

\begin{figure}[H]
    \centering
    \includegraphics[width=10cm,height=6cm,keepaspectratio]{Resources/hover_net_example/panoptic_final.PNG}
    \caption{Predicted Panoptic Mask (Instance + Type) Overlayed on top of Original}%
    \label{fig:hovernet_instance_seg}%
\end{figure}
%I observed that long nuclei are prone to \textbf{over-segmentation}\footnote{The opposite of under-segmentation where a single segment is instead predicted as multiple.} because they contain not a single
\section{Cell Graph Construction}
Histopathological graphs \cite{ahmedt-aristizabalSurveyGraphBasedDeep2021} require three components to be defined: the entities being modelled, the node embeddings, and the edges. Cell graphs constrain the entity being modelled to cells, leaving node embeddings and edges free for us to specify. I do so now, taking inspiration from \cite{deepakanandHistographsGraphsHistopathology2020}:

\subsection{Node Embeddings}
For each identified nucleus, I take a \textbf{64x64 crop} encompassing it. From this crop, I extract a series of morphological and biological features described below:
\begin{itemize}
    \item \textbf{Cell Type}: I store a one-hot encoding of the type of cell identified in \S \ref{sec:nucleus_type}. This contributes 5-dimensions.
    
%    \item \textbf{Average RGB Value}: The average colour across the crop is calculated. This gives the model information about both what stain vectors are present, and in with what intensity. This contributes 3-dimensions.
    
    \item \textbf{Gray Level Co-occurence Matrix (GLCM)}\cite{haralick1973textural}: The GLCM captures textural information about an image. To compute the GLCM, the image is first converted to gray-scale, and its values are quantised into $n$ levels. The GLCM is an $n \times n$ matrix which counts how many times a pair of pixels of certain quanta appear in the image. These pairs are taken at each pixel $(x,y)$ and at a constant offset $(x + \Delta x, y + \Delta y)$. Hence, different quantisations and offsets define different GLCMs. I take two GLCMs at $n=5$, one with horizontal offset $(\Delta x, \Delta y) = (1,0)$ and one with vertical offset $(\Delta x, \Delta y) = (0,1)$. This contributes 50-dimensions.
    
    
    % TODO Do I need to elaborate?
    \item \textbf{ResNet-50 Features}: The intermediate layers of a CNN can be useful for encoding morphological features; \S \ref{sec:convolutions} highlighted that edge and corner primitives were identified in the earlier layers of a CNN. By training an autoencoder (\S \ref{sec:auto_encoders}) with a ResNet-50 backbone, I was able to train such a CNN to encode meaningful morphological features. The layer selected returns a $16 \times 16 \times 256$ dimensional vector; the $16 \times 16$ comes from a two downsamplings of the $64 \times 64$ crop, and $256$ is the number of feature maps. This vector is further reduced by global average pooling each feature map. The final vector therefore contributes 256 dimensions to the node-embedding
    
    
    \item \textbf{Number of Neighbours}: The number of nuclei that are within a 100 pixel radius are computed. This contributes 1-dimension.
\end{itemize}

The final node-embedding is made by concatenating the above features together, yielding a 312-dimensional vector.

% TODO image depicting this vector
\subsection{Edge Definitions}
I opted for a K-Nearest Neighbours (KNN) based graph \cite{eppstein1997nearest}. Two nodes $a$ \& $b$ are connected if, in terms of pixels, $b$ is among the k-th closest nodes to $a$. Specifically, I chose \textit{k} to be 6 as it struck a good balance between sparsity and density. The choice of KNN as a graph definition is discussed in \S \ref{sec:eval_knn}.

Below is the graph for the running example (Figure \ref{fig:b002}), where the nodes are represented by the image crop from which the embeddings will be generated from:


\begin{figure}[H]
    \centering
    \includegraphics[height=8cm,keepaspectratio]{Resources/cell_graph.PNG}
    \caption{A visualisation of the cell graph of Figure \ref{fig:b002}}
    \label{fig:cell_graph_crops}
\end{figure}


\section{Graph Classification with GCN}
In order to classify cell graphs, and hence H\&E images, a GNN was used. A variety of architectural setups were experimented, including GINTopK \cite{wang2021cell} which diagnosed gastric cancer. It was difficult to translate the success of existing models to my project because of their reliance on the underlying graph definition. The most effective architecture, and the one used in the end, was based on the \textbf{Graph Convolution Network} or \textbf{GCN} \cite{kipf2016semi}. In this section, I explain the GCN layer, and outline the full architecture and training of the model. 

\subsection{Architecture}
\subsubsection{Convolutions}

The GCN layer is a simple graph convolution layer, and is particularly effective when applied to homophilic graphs; that is to say graphs where neighbouring nodes associate strongly with one another. Because of the biological signalling that occurs between adjacent cells, it is natural to assume some degree of homophily in cell graphs.

To explain how the GCN layer works, I use the message passing framework mentioned in \S \ref{sec:graph_convolution}. Messages are constructed by multiplying neighbouring node embeddings by $c_{ij} =\frac{A(x_i,x_j)}{\sqrt{d(x_i)d(x_j)}}$. $A(x_i,x_j)$ is the edge weight between node $i$ and $j$ (set to 1), and $d(x) = 1+\sum_{y\in N(x)}A(x,y)$. One can interpret $c_{ij}$ as a normalised or relative importance between neighbours, which amplifies or dampens the message, namely the node embedding of said neighbour. The aggregator is addition, and $\phi$ is computed with an MLP.

$$ h_i = {\text{MLP}}\left(\sum_{x_j\in {N(x_i)\cup \{x_i\}}}c_{ij}x_j\right)$$

The convolution layer serves two purposes: 1) To propagate information between nodes, and 2) to learn a better representation of cells based on that information. The second of these responsibilities is handled by the MLP whose complexity determines how expressive the intermediate node embeddings will be. Instead of using the default single linear layer, I use a two-layer MLP with batch normalisation and ReLU activation:


\begin{figure}[H]
    \centering
    \includegraphics[width=14cm,height=10cm,keepaspectratio]{Resources/gcn_layer.png}
    \label{fig:gcn_layer}
    \caption{A GCN convolution followed by a two layer MLP}
\end{figure}

In the figure above, the linear layer of the GCN has been moved to the MLP for clarity. This way, the GCN only performs a weighted sum of neighbouring node embeddings.

\subsubsection{Global Pooling and Prediction}
Global pooling layers are aggregators of nodes, and the choice of aggregation will depend on what properties are useful for differentiating between graph classes \cite{xu2018powerful}: mean pooling learns about node distributions, while max pooling learns about sets of nodes with distinct elements. 

Cancer is recognised by deviation from normality in cells, and hence mean pooling would be applicable. Equally, cancerous tumours can form in close proximity to healthy tissue, and so the presence of cancer can be identified by the presence of certain cells, making max pooling a suitable candidate. It is for this reason that I use both \textbf{max} \& \textbf{mean pooling}.

After passing the graph through \textbf{seven} convolution layers, a global max and mean pool is taken, the outputs are concatenated, and then fed into an MLP that will predict if cancer is present. The entire architecture is visualised below:

\begin{figure}[H]
    \centering
    \includegraphics[width=14cm,height=10cm,keepaspectratio]{Resources/GCN_model.png}
    \label{fig:gcn_layer}
    \caption{The full cell graph model}
\end{figure}

\subsection{Training}
\subsubsection{Data Preparation and Augmentation}
I trained the GNN with the BACH dataset. Recall that the \textbf{BACH} consists of 400 H\&E images spanning four classes, two cancerous and two non-cancerous. Before training, the images are fed through the first three pipeline steps, namely \textbf{stain normalisation}, \textbf{nuclei segmentation} and \textbf{graph construction}. The results are then collated in storage to form an artificial dataset.

In order to extend the dataset, I performed a simple graph augmentation. As a training graph is fetched from storage, the locations of the nodes are shifted by a random amount (no more than 20 pixels). Edges have to be recalculated as the KNN post condition is violated. In this way, new edges are formed and force messages to take different paths during graph convoluting. 


\subsubsection{Loss Function}
 Cross entropy loss, already mentioned in \S \ref{sec:loss_hover}, was used for multiclass classification. For completeness I outline how it is computed: The output of the MLP is fed into a \textbf{softmax} layer. This makes the outputs sum to one and therefore have a probabilistic interpretation.

$$\hat{p_i} = \text{softmax}(x_i,\bar{x}) \triangleq \frac{\exp{x_i}}{\sum_{x_j \in \bar{x}} \exp{x_j}}$$

Logarithms are taken over the reciprocal of the predicted probabilities and are then multiplied by the true probabilities (which is 1 for the true class and 0 for the rest). 
$$\mathcal{L} = \sum_{c \in \{\text{N,B,In,Iv}\}} {p_c log(\frac{1}{\hat{p_c}})} $$

\subsubsection{Regularization}
Learned models need to be robust and generalise to unseen data. For small datasets, there is a tendency for the model to \textbf{overfit} to the training data and it will therefore perform significantly worse on the test set. This happens in part because the model is too complex and is attempting to capture noise in its predictions.

\textbf{Regularization} is the process by which we artificially make models simpler. The closer a parameter is to zero, (typically) the smaller its contribution will be to the model so much so that it can be eliminated from equations. By penalizing models with large weights, we are effectively forcing only the most important relations to be learned.

I made use of two types of regularization: \textbf{weight decay} and \textbf{dropout}. \begin{itemize}
    \item Weight decay is an optimizer hyperparameter that reduces the magnitude of the current weights at each step. It was set to 1e-3.
    \item Dropout is a type of layer that blocks a random subset of input signals\footnote{When evaluating, dropout is ignored}. In doing so, the model is forced to distribute its reasoning among all neurons as opposed to just a single. I used a dropout layer in the final MLP, and set the percentage of nodes to be dropped to 40\%. 
\end{itemize}

In addition, I intentionally constrained the width of the network to 32, compared to 256 in \cite{wang2021cell}. Such a width requires at least 64x more parameters than my model, and with only 300 graphs to train from, this would have been infeasible.


\section{GCExplainer}
\textbf{GNNExplainer} \cite{ying2019gnnexplainer}, a prominent example of post-hoc explainbility\footnote{Frameworks that make use of trained models instead of needing to be incorporated into the actual architecture.}, produces local explanations to justify model predictions. This means explanations are specific to that particular example and do not originate from some prior understanding of the task; it is left to the user to draw meaningful connections, and this is susceptible to confirmation bias \cite{adebayo2018sanity}. \textbf{GCExplainer}\cite{magister2021gcexplainer} instead generates global explanations for GNNs by discovering and recognising concepts.

Concepts are high-level units of information used to reason about the data. For example, a car can be differentiated from a cat by the presence of wheels (a high level unit) but not necessarily by colour (a low level unit). Medical practitioners will communicate their decisions in terms of these concepts, pulling from a rich repository of prior categorised concepts; the discussion in \S \ref{sec:cancer_stages} on cancer demonstrated such reasoning. Concepts need to span and pervade the dataset in order for them to be applicable to new examples.

The hypothesis is that, where humans reason explicitly in terms of concepts, the deep learning models reasons implicitly in terms of them because concepts can be effective indicators for predicting. I will now explain how GCExplainer automatically infers concepts from the training set, how they can be communicated to the user, and finally how they can be used to explain predictions.

% How are concepts detected
\subsection{Concept Detection}
After all the graph convolutions, nodes embeddings are mapped to a meaningful intermediate space. We hypothesise that this space is a space of concept representations, and nodes which are mapped near each other are likely to be part of the same concept. 

Clustering is therefore the primary ingredient for concept discovery, and \textbf{K-Means} is used to achieve this. By recording the final convolution's node activations and clustering with K-Means, \textit{k} concept representations are learned. Assigning nodes to concepts is a matter of assigning their activation embedding to the nearest concept representation. 

\begin{figure}[H]
    \centering
    \subfloat[\centering]{{\includegraphics[width=10cm,height=6cm,keepaspectratio]{Resources/k6.PNG} }}%
    \qquad
    \subfloat[\centering]{{\includegraphics[width=10cm,height=6cm,keepaspectratio]{Resources/k60.PNG} }}%
    \caption{(a) k=8, (b) k=60}%
    \label{fig:concepts_space}%
\end{figure}

By performing dimensionality reduction on the activations with t-SNE \cite{van2008visualizing}, one can visualise the concept clusters on a 2-D plot as I have done above.

The natural next question is what value of \textit{k} should be chosen. Too small and distinguishing concepts get merged. Too large and concepts become specific only to a very small percentage of graphs. The original paper offers \textit{k} to be selected by domain experts but due to a lack of time this was not possible. I set \textit{k} to be 32 with justification left to the evaluation.

% How are they communicated
\subsection{Concept Representation}
So far, the discovery of concepts has based on individual nodes, but what we are looking for is a more macroscopic unit to represent concepts. Concepts should take the modality of the underlying data strucutre which would imply that subgraphs should be used to represent concepts. Magister \cite{magister2021gcexplainer} suggests selecting those nodes closest to the cluster centroid and then taking the \textit{n}-hop neighbourhood around them. The advantage of this approach is that it again includes human agents in the decision making process in order to select the value for \textit{n}. In this project, I experimented with another representation definition. Again, find the nodes which are closest to the cluster centroid, but instead take the surrounding subgraph formed by connecting nodes of the same concept.



\begin{figure}[H]
    \centering
    \includegraphics[width=10cm,height=12cm,keepaspectratio]{Resources/concept_graph_b002.PNG}
    \caption{Nodes in a single cell graph coloured by concept. Same examples as Figure \ref{fig:b002}}%
    \label{fig:concept_graph}%
\end{figure}
\squeezeup

To illustrate this, observe the above cell graph coloured by the concept of its nodes. By dissecting this graph by colour - that is to remove all edges between different coloured nodes -  a set of candidate subgraphs is generated. After looking at candidates across the entire dataset and comparing them based on how close their nodes are to the cluster centroid, the top-3 most representative subgraphs can be found.

In general, it is challenging to give convincing and interpretable examples by displaying the raw mathematical graph. Fortunately, the cell graphs are derived from an H\&E image, and realigning the graph on top of the image allows us to pictorially represent the concepts. Each node is placed on the cell it encodes and a convex hull is taken to encompass the entire concept; this is further padded for clarity.

I now present some of the concepts discovered across the training set, their top-3 representations, and give an interpretation for each: 
{

\label{sec:concept_interpretation}
\begin{itemize}
    \item \textbf{Concept 6}) Epithelial cells lining benign tissue.
\end{itemize}

\vspace{-25pt}

    \begin{figure}[H]
  \begin{subfigure}{.3\linewidth}
    \centering
    \includegraphics[width = \linewidth]{Resources/concepts/c6e0.png}
  \end{subfigure}%
  \hspace{1em}% Space between image A and B
  \begin{subfigure}{.3\linewidth}
    \centering
    \includegraphics[width = \linewidth]{Resources/concepts/c6e1.png}
  \end{subfigure}%
  \hspace{1em}% Space between image B and C
  \begin{subfigure}{.3\linewidth}
    \centering
    \includegraphics[width = \linewidth]{Resources/concepts/c6e2.png}
  \end{subfigure}

    \centering

    \label{fig:concept_6}%
\end{figure}

\vspace{-25pt}

\begin{itemize}
    \item \textbf{Concept 30}) Dysplastic connective cells in cancerous tissue. Shape of nuclei are very irregular.
\end{itemize}    

\vspace{-25pt}

    \begin{figure}[H]
  \begin{subfigure}{.3\linewidth}
    \centering
    \includegraphics[height=5cm,keepaspectratio]{Resources/concepts/c30e0.png}
  \end{subfigure}%
  \hspace{1em}% Space between image A and B
  \begin{subfigure}{.3\linewidth}
    \centering
    \includegraphics[height=5cm,keepaspectratio]{Resources/concepts/c30e1.png}
  \end{subfigure}%
  \hspace{1em}% Space between image B and C
  \begin{subfigure}{.3\linewidth}
    \centering
    \includegraphics[height=5cm,keepaspectratio]{Resources/concepts/c30e2.png}
  \end{subfigure}

    \centering


    \label{fig:concept_30}%
\end{figure}    


\begin{itemize}
    \item \textbf{Concept 31}) Healthy cells in normal tissue. Regular, honeycomb-like organisation.

\vspace{-20pt}
    \begin{figure}[H]
  \begin{subfigure}{.3\linewidth}
    \centering
    \includegraphics[height=5cm,keepaspectratio]{Resources/concepts/c31e0.png}
  \end{subfigure}%
  \hspace{1em}% Space between image A and B
  \begin{subfigure}{.3\linewidth}
    \centering
    \includegraphics[height=5cm,keepaspectratio]{Resources/concepts/c31e1.png}
  \end{subfigure}%
  \hspace{1em}% Space between image B and C
  \begin{subfigure}{.3\linewidth}
    \centering
    \includegraphics[height=5cm,keepaspectratio]{Resources/concepts/c31e2.png}
  \end{subfigure}

    \centering

    \label{fig:concept_31}%
\end{figure}    
\end{itemize}
}


\vspace{-20pt}
% Explaining a prediction
\subsection{Explaining a Prediction}
Now that concepts have been identified and can be communicated to the pathologist, all that remains is to explain new predictions based on the discovered concepts. After dissecting the concept graph, the concept which maximises $P(\text{predicted class} |\text{concept})$ is selected as the supporting evidence. This conditional probability is approximated using the joint frequency distribution of class to concept. Below is an illustrating example\footnote{This image was by accident taken from the training set, and I only realised at the end. This figure is not intended to demonstrate the predictive power of the model, but instead the ability to explain.} where the likeness of segments to benign epithelial cells used for lining (concept 6) is being chosen as evidence:  
\begin{figure}[H]
    \centering
    \includegraphics[width=17cm,height=10cm,keepaspectratio]{Resources/explanation_for_b002.PNG}
    \caption{Explanation for prediction of Figure \ref{fig:b002}. The concepts depicted on the right do not originate from the image, but instead from different samples exhibiting the same concept.}%
    \label{fig:concept_graph}%
\end{figure}


\vspace{-20pt}
\section{Repository Overview}
\vspace{-10pt}
I present the project directory structure at a glance. All the work culminates in the \texttt{predict\_cancer.py} program that performs all the steps in Figure \ref{fig:full_overview}. Note, the actual datasets live within the top \texttt{data} folder, while the programs for interfacing with this data are stored in \texttt{src > datasets}. 
\begin{figure}
\centering
\begin{forest}
  for tree={folder,grow'=0,fit=band,inner sep=0.1}
  [\faFolderOpen \hspace{3pt} XAI-Cancer-Diagnosis
    [\faFolderOpen \hspace{3pt} data
    ]
    [\faFolderOpen \hspace{3pt} notebooks]
    [\faFolderOpen \hspace{3pt} src
        [\faFolderOpen \hspace{3pt} datasets
            [\Python \hspace{3pt} BACH.py]
            [\Python \hspace{3pt} PanNuke.py]
        ]
        [\faFolderOpen \hspace{3pt} deep\_learning
            [\faFolderOpen \hspace{3pt} architectures]
            [\faFolderOpen \hspace{3pt} metrics]
            [\faFolderOpen \hspace{3pt} trainers]
            [\faFolderOpen \hspace{3pt} explainability]
        ]
        [\faFolderOpen \hspace{3pt} scripts]
        [\faFolderOpen \hspace{3pt} transforms 
            [\faFolderOpen \hspace{3pt} cell\_segmentation
                [\Python \hspace{3pt} hovernet\_post\_processing.py]
            ]
            [\faFolderOpen \hspace{3pt} graph\_construction
                [\Python \hspace{3pt} graph\_extractor.py]
                [\Python \hspace{3pt} node\_embedding.py]
            ]
            [\faFolderOpen \hspace{3pt} image\_processing
                [\Python \hspace{3pt} filters.py]
                [\Python \hspace{3pt} he\_normalize.py]
            ]
        ]
        [\faFolderOpen \hspace{3pt} utilities]
        [\faFolderOpen \hspace{3pt} vizualiations]
        [\Python \hspace{3pt} predict\_cancer.py]
    ]
    [\faFolderOpen \hspace{3pt} tests]
  ]
\end{forest}
\caption{The salient part of the project directory}
\end{figure}


%The name GINTopK refers to the convolutional  and local pooling layers used, namely GIN \cite{xu2018powerful} and Top-k \cite{cangea2018towards} respectively.

%\subsubsection{GIN}
%The Graph Isomorphism Network or GIN is an expressive graph convolutional layer, comparable with the Weisfeiler-Lehman test for graph isomorphism \cite{weisfeiler1968reduction}. In other words, it has the capacity to distinguish between a broad class of graphs.

%To compute the GIN layer for a particular node, the embeddings of its neighbours and itself are summed together, and then passed through a MLP:

%$$h_i = \text{MLP}_{\theta}\left((1+\epsilon)x_i + \sum_{x_j \in \mathcal{N}(x_i)} x_j \right)$$

%The $\epsilon$ term, which contributed more expressivity to the model, is set to zero in my configuration. I also chose to use a single pre-activated linear layer as my MLP:




%\subsubsection{Top-K Pooling}
%Top-K pooling achieves hierarchical pooling by keeping only the k\% most important nodes. The ``importance'' of a node is computed via a learnable function $f$ that assigns a score to each node.


%\subsubsection{Full Architecture}
%A ``block'' consists of two GIN layers followed by a Top-K layer, and these blocks are sequenced one after another. As the graph arrives at the end of a block, the output is then separately \textbf{global average pooled}, with this vector being stored in a list of \textbf{readouts}. Once the graph has passed through all blocks, the readouts are all concatenated together and fed through a MLP. 

%\begin{figure}[H]
 %   \centering
%    \includegraphics[width=10cm,height=6cm,keepaspectratio]{Resources/GINTopK.png}
%    \caption{My Configuration of GINTopK. The term ``Readout'' denotes a global average pooling}
%    \label{fig:gintopk}
%\end{figure}

%My architecture configuration uses two blocks, and also an MLP of depth two.

==> chapters/intro.tex <==
\setcounter{page}{1}
% Construction of a cell graph (what a cell graph is) used for predicting cancer. Post hoc explainability applied afterwards.
\textit{
merging GCExplainer and LEN?
The Len could output observations on the state of the cell and tissues (such inflammation, vascularisation, innervation, etc) useful for doctors
This coupling could make it more new.
The aim of my project is to develop a complete pipeline for diagnosing cancer using deep learning. As well as being able to generalise to unseen data, my AI model explains predictions, which is an essential requirement for clinical settings.}

\textit{In this chapter, I outline the motivation and challenges for such a project, and give a short survey of previous work.}


\section{Motivation}
% Its cost on lives, financial cost 
Cancer is a leading cause of death worldwide. It accounted for nearly 10 million deaths globally in 2020 \cite{who:cancer}. With an aging population, the prevalence of cancer will only increase \cite{increase_cancer}, so work in the area of diagnosis and treatment is of the upmost importance.

Early diagnosis is critical for maximising chances of a successful treatment, which ultimately saves lives and reduces financial costs on society. Artificial Intelligence (AI) for digital histopathology\footnote{The study of disease at a cellular level.} is revolutionising the field by efficiently and accurately diagnosing cancer \cite{forondaAIRevolutionCancer2020}; This has been accelerated by advancements in computer vision and an increase in the amount of digitized clinical data.
% The field of Digital pathology and its contribution to pathologists
    %includes the process of digitizing histopathology, immunohistochemistry or cytology slides using whole-slide scanners as well as the interpretation, management, and analysis of these digitized whole-slide images using computational approaches.
% The success of computer vision and deep learning to the field

\section{Challenges}
% The black box nature of these trained systems. Lack of trust by doctors. Final hurdle. Mentioned CACM article
In slew of all their advances, Artificial Intelligence models fail to gather significant adoption by medical practitioners. Some \cite{kundu2021ai} have pointed to the ``black-box'' nature of these models as the limiting factor; models are fed an input and, as if by some inscrutable magic, come to a decision. When placed in a high stakes environment like a hospital, doctors want such models to instil confidence not doubt. It is for this reason that the final hurdle in the way of attaining widespread utility is the challenge of explainable AI \textbf{(XAI)}, in my opinion. 

% "Clinical Wild" Real world problem

\section{Previous Work}
Convolutional Neural Networks (CNN) are a particular AI model that operates over images. They have already achieved noteworthy success in the medical field, for example in the analysis of head MRIs in order to identify Alzheimer's disease \cite{lin2018convolutional}.

At the other end of the deep learning spectrum, Graph Neural Networks (GNN) have seen a resurgence in popularity. They were originally proposed by Scarselli \cite{scarselli} in 2008 and have been pulled in many different directions since \cite{kipf2016semi,velivckovic2017graph,gilmer2017neural}.

Networks are present at all levels of biological abstraction \cite{zhang2014network}, from ecological food webs to the brain, to the signaling networks between cells. Cells are synergistic, and their function is dictated by their context - the relative location of the cell within the surrounding tissue. By disturbing this structure, the tissue may no longer be able to fulfil its role, and this can have global repercussions. An example of this can be seen in emphysema, a disease of the lungs often caused by smoking \cite{gartner2012color}. Here, the alveolar walls are damaged and this change in tissue structure leads to a reduction in both lung elasticity and the available area for gas exchange, posing a threat to the respiratory system. Similarly, cancer can also be detected at the cellular level by observing a change in the structure and composition of tissue:


\begin{figure}[H]
        \centering
        \includegraphics[width=14cm,height=10cm,keepaspectratio]{Resources/structural deviation.png}
        \caption{A cellular comparison of the bladder between healthy and cancerous tissue. The healthy tissue has an ordered and clear structure, while the cancerous tissue signficantly deviates from this. Taken from \cite{chen2018relationship}.}
        \label{fig:structural_deviation}
\end{figure}

It is natural to represent these structures with a mathematical graph, and for this reason Graph Neural Networks are now being chosen as the bedrock of cancer diagnosis projects over Convolutional Neural Networks. \cite{ahmedt-aristizabalSurveyGraphBasedDeep2021} gives a survey of Graph Neural Networks for computational histopathology, and I point to HACT-Net \cite{patiHierarchicalGraphRepresentations2021} as a significant example.

\section{Project Overview}
At a high level, my project examines three steps:
\begin{enumerate}
    \item To construct biological graphs from an image using a CNN.
    \item To predict cancer from these graphs with a GNN.
    \item To explain the predictions.
\end{enumerate}

\begin{figure}[H]
        \centering
        \includegraphics[width=14cm,height=10cm,keepaspectratio]{Resources/coarse_overview.png}
        \caption{High level project overview}
        \label{fig:coarse_overview}
\end{figure}

==> chapters/preperation.tex <==
\textit{In this chapter, I present the relevant theory and research in computational pathology and deep learning. In the first half I discuss: the biological components of cancer and the apparatus used for making observations, classical and deep learning approaches to the task of instance segmentation, graph neural networks, and an overview of Explainable AI. In the second half, I document the requirements of my project and relevant tooling I used.}

\section{Computational Pathology}
    \subsection{Types of Cells}
    % H&E histological images and how to detect below:
        % Types of cells
                % Check PanNuke for types
            % Epithelial Cells - Neo vs Non Neoplastic
            % Connective Soft Tissue - Fibroblastc - fibers - endothelial
Multi-cellular organisms are composed of a series of systems (e.g. respiratory, nervous), which in turn are composed of organs, then tissues, then cells. Although composition differs among tissue types, there is overlap in the types of cells present; Hence an understanding of their roles is useful irrespective of the task. I consider the taxonomy presented in \cite{gamperPanNukeDatasetExtension2020}. They define two main categories - \textbf{neoplastic} and \textbf{non-neoplastic} cells. They further break down non-neoplastic cells into 4 more categories, giving 5 categories in total described below:
\begin{itemize}
    \item \textbf{Neoplastic Cells}: meaning `new growth', this class includes both benign and malignant tumours. The type of tumour depends on what its original cell was. In most breast cancers, the tumour is a carcinoma, originating from epithelial cells.
    \item \textbf{Non-neoplastic Epithelial Cells}: these cells form a protective lining around tissues.
    \item \textbf{Inflammatory Cells}: part of the immune system, this class includes white blood cells (macrophages and leukocytes) and the cells that produce them (lymphoid cells). Their presence is therefore an indicator for disease.
    \item \textbf{Connective Cells}: the most common subtype in this class are fibroblasts. They provide the structural framework of tissue (called the \textbf{stroma}) by synthesizing \textbf{collagen} and the \textbf{extracellular matrix}\footnote{An interlocking mesh of proteins and biochemicals}.
    \item \textbf{Dead Cells}
\end{itemize}
% TODO Images of the 5 cells types from Pietro's book

% TODO COMPILE TOGETHER
    \subsection{Cancer}
    \label{sec:cancer_stages}
    %What is cancer?
    Cancer is a group of diseases that cause uncontrolled division of abnormal cells. Because of the breadth of diseases encompassed by cancer, the causes and symptoms vary. The most common form of cancer is breast cancer, which effects 1 in 8 women in their lifetime \cite{nhs_choices}.
    
    
    %Stages of cancer
    Cancer is a gradual process, and its development is divided into stages:
    \begin{itemize}
        \item \textbf{Normal}: Tissue is healthy.
        \item \textbf{Pre-Malignant / Dysplasia}: Cells undergo a series of abnormal morphological changes, such as enlargement (hypertrophy), excessive multiplying (hyperplasia), or irregularities in shape. Dysplasia is not cancerous, but it is possible for dysplastic cells to become cancerous.
        \item \textbf{Malignant}: The tumour has become problematic and should be removed. If the cancer has spread and \textbf{invaded}  other parts of the body, it is said to have ``metastasized'' and this makes it very difficult to treat. If, however, the cancer has not spread and remains \textbf{in situ}, then this gives more options for handling the prognosis.
        
    \end{itemize}
    
    There are both cellular and inter-cellular indicators of cancer. I now give a short example of both:
\begin{itemize}
    \item The Gleason score is a standard for scoring prostate cancer and is determined by looking at the dissimilarity of cancer cells from normal prostate cells.
    \item The ``neighbourhood'' in which cells reside is called the \textbf{microenvironment}, and is believed to have significant role in the development of tumours \cite{fane_weeraratna_2020}. Connective cells, immune cells and signalling molecules (like hormones) make up the microenvironment, and abnormalities in this composition may point towards cancer.
\end{itemize}
    
    
    % What is cancer in detail.
    % Stages of cancer
        % Invasive vs Insitu
    % Cellular Characteristics
        %Dysplasia
        %Gleason Scorehttps://www.overleaf.com/project/6241b22d35f6dc19b22e9f82
    % Importance of the microenvironment
    
    
    
    \subsection{H\&E Staining}
    Tissue samples are stained to extract information about particular organelles, smaller biological sub-units within a cell that perform a certain task. The chemicals used have affinities for particular biological substances so that, when illuminated and observed under a microscope, areas with a high density of that substance will be dark and areas with a low density will be light. \textbf{Hematoxylin} stains RNA and DNA dark purple, highlighting the nucleus. \textbf{Eosin} stains proteins pink which highlights the cytoplasm and extracellular matrix. Together, they form the \textbf{H\&E stains} which is a gold standard in histopathology.
    
    % Problems with the procedure
    H\&E staining is a cheap and quick procedure. However, H\&E dyes are not standardised \cite{schulte1991standardization}. Furthermore,  using inconsistent proportions of the two dyes or leaving samples in the chemical for too long can cause variability in stain intensity. \textbf{Stain normalisation} aims to rectify this and is discussed in \S \ref{sec:stain_norm}.
        
    % Importance for later stages 
    
    %Insert photograph with caption Of single Image


    \begin{figure}[H]
        \centering
        \includegraphics[width=14cm,height=6cm,keepaspectratio]{Resources/b002.PNG}
        \caption{Example of an H\&E image from \cite{aresta2019bach}}
        \label{fig:b002}
    \end{figure}
    
    %Insert several photos showing range
    
    
    
    \subsection{Cell Graph}

    H\&E images implicitly encode the structural information present in tissue. By representing cells as nodes and edges as relations between them, a tissue's structure can instead be explicitly coded for. This concept was first proposed by Yener et al. \cite{yener2016cell} in what they called the ``cell graph''.
    
    In order to create the cell graph, each cell must first be identified. Since each cell contains a single nucleus, searching for nuclei serves as an effective proxy for detecting cells; this can be accomplished with \textbf{instance segmentation}.
    
\section{Segmentation}
\begin{definition}{\textbf{Segmentation}}. The goal is to find a function $f$ that maps each pixel to a particular class $\in C$: 
$$f:\mathcal{R}^{3\times \text{width} \times \text{height}} \rightarrow C^{\text{width} \times \text{height}}$$

Adjacent pixels with the same assigned class are part of the same segment.
\end{definition}

%TODO: TWEAK
There are three types of segmentation:
\begin{itemize}
    \item \textbf{Semantic Segmentation:} $C$ stores the category of the segment, e.g. person, car or background. Where objects of the same category overlap, the same segment will span both of them.
    \item \textbf{Instance Segmentation:} $C$ stores ids for each object. Overlapping objects can be differentiated but their category cannot be inferred, unless there is only one category of interest (+ background).
    \item \textbf{Panoptic Segmentation:} $C$ stores both id and category of each segment.
    
\end{itemize}

    \begin{figure}[H]
        \centering
        \includegraphics[width=14cm,height=6cm,keepaspectratio]{Resources/segmentation types.png}
        \caption{Types of segmentation. Figure from \cite{segmentation_types}}
        \label{fig:seg_types}
    \end{figure}

The task of segmentation falls under the umbrella of \textbf{computer vision}. Methods in this field are often divided into classical and neural approaches. I give a brief discussion of classical approaches to segmentation below, and leave an introduction of neural approaches to section \ref{sec:CNN}.



Classical approaches can be further divided into three types of methods\footnote{See \cite{glasby_horgan} for a more comprehensive overview.}:
\begin{itemize}
    \item \textbf{Thresholding / Pixel Based Segmentation:} Classes are assigned based on where a pixel lies on the range of possible values. A popular algorithm for automatically determining decision boundaries is \textbf{Otsu's method} \cite{otsu}, analogous to k-means on the image's intensity histogram \cite{otsu-kmeans}.
    \item \textbf{Region Based Segmentation:} Pixels are iteratively grouped together based on similarity with neighbouring pixels. The \textbf{watershedding} algorithm is such an example and is described in section \ref{sec:watershedding}.
    \item \textbf{Edge Based Segmentation:} Using edge detection filters like \textbf{Prewitt} \cite{prewitt1970object} and \textbf{Sobel} \cite{sobel1990isotropic}, the boundaries of segment regions can be discovered. See section \ref{sec:CNN} for an elaboration on filters.
\end{itemize}

In practise, these methods are not mutually exclusive and can be used in combination.

\section{Geometric Deep Learning}
\textit{My project makes extensive use of deep learning models, which is why I think it is worthwhile to explore the associated theory. I begin by showing deep learning's place in artificial intelligence and the mathematical framework that it resides in. I then highlight the formidable curse of dimensionality and point to geometric deep learning as a modern solution to it. I finally turn to Convolutional and Graph Neural Networks as my used examples of geometric learning.}

\subsection{Machine Learning}
A subfield of AI, machine learning (ML) studies algorithms that improve performance on a task with experience and data \cite{mitchell1997machine}. The most successful class of algorithm is supervised algorithms where the computer has examples of input-output pairs and tries to infer the mapping which best explains the observations\footnote{I will refer to the input space as $X$, the output space as $Y$, and the mapping as a function from $X \rightarrow Y$}. When the output space $Y$ is \textbf{continuous} (like temperature or people's heights), the task is referred to as \textbf{regression}, as opposed to outputs that are \textbf{discrete} (like dog breed or nationality), where the task is referred to as \textbf{classification}. ML is chosen in situations where the functional relationship is too complicated to express classically (like human vision), and for which an inferred approximation will suffice.

Most supervised approaches share the same framework for learning, and contain the following key components:
\begin{itemize}
    \item \textbf{Parametric Model}: This is a mathematical function $f:W\times X\rightarrow Y$, which when given parameters $w$, yields a specific function $f(x;w): X \rightarrow Y$. Below are some examples of parametric models:
    \begin{itemize}
        \item  \textbf{Linear Models}: $f(\bar{x};w)\triangleq \sum{w_i x_i}$.
        \item \textbf{Linear Models with Activation Function}: $f(\bar{x};w) \triangleq \sigma(\sum{w_i x_i})$. $\sigma$ is the \textbf{activation function} and its purpose is to introduce non-linearity into the computation. A historically significant example is the \textbf{Perceptron\cite{rosenblatt1958perceptron}}  whose activation function was the \textbf{step} function.
    \end{itemize} 
    %By considering $m$ perceptrons, we can try learning mappings of input vectors from $R^n\rightarrow R^m$.
    
    \item \textbf{Dataset}: A set $(X\times Y)^n$ of $n$ labelled observations (in the sense that each input is paired with a target output). It is standard practise to partition the dataset in advance into \textbf{training} and \textbf{test} sets; the former being used in the learning algorithm and the later being used to evaluate the generalizability of the learned model. 
    
    \item \textbf{Loss Function}: This is a function $E:(Y \times Y) \rightarrow \mathcal{R}$ that measures ``how good" a prediction is. Namely for a single observation $(x,y)$, the loss is $E(y,\hat{y})$, where $\hat{y}$ is the prediction $f(x;w)$. The lower the loss, the better the prediction. Common loss functions include the \textbf{square of errors} ($E(y,\hat{y}) \triangleq ||y-\hat{y}||_2^2$) for regression and \textbf{cross-entropy} for classification.
    
    \item \textbf{Learner}: This is the function $L:(X \times Y)^n \rightarrow W$ which figures out the best possible parameters (and hence function) to explain the observations. A popular class of learning algorithms are those that try to find parameters $\hat{w}$ that \textbf{minimises the empirical risk} (roughly the average loss across the training set):
    $$\hat{w}=\argmin_{w}\frac{1}{n}\sum_{(x,y)\in (X\times Y)^n}{E(y,f(x;w))}$$
    Since the empirical risk is a function of the parameters, the learner can be seen as searching for a minima in parameter space. It is for this reason that machine learning concerns itself with the study of optimization.
    
    
\end{itemize}




% Extension to Deep Learning - more complex models (dense - universal approximation). Perceptron, def of DL in GOodfellow


\subsection{Deep Learning}
This subdiscipline of machine learning is interested in stacking layers of simple parametric functions so that more complex functions can be represented.

The components of supervised learning apply here, but often are known under different guises. In particular:
\begin{itemize}
    \item \textbf{Architecture (for the Parametric Model)}: this refers to the specification of what layers are used and how they are composed. For example, a \textbf{linear layer} is made by horizontally stacking $m$ linear models (each $\mathcal{R}^n\rightarrow \mathcal{R}$) to get a function $R^n \rightarrow R^m$, and an \textbf{activation layer} is made by applying the same activation function to each of the outputs of the previous layer. By interleaving linear and activation layers, one gets a \textbf{multilayered perceptron (MLP)}\footnote{Also called a feed forward network or artificial neural network.}.
    \item \textbf{Optimizer (as part of the Learner)}: Deep learning architectures virtually always define a differentiable functon in terms of their weights. As such, the loss function is also differentiable, and by moving in the direction of steepest descent, one can iteratively decrease empirical risk; this is called \textbf{gradient descent}, because the direction of steepest descent is ``minus the derivative of empirical risk".
    
    It is often helpful imagining the loss function as defining a surface in parameter space, and gradient descent as dropping a marble to find the bottom of this terrain. Such an analogy also illuminates the challenges with optimizing this way. Firstly, how far do you step at each iteration? Too short and you don't make any progress. Too long and you may jump over the valley. Luckily, we have some control over this through a hyperparameter called the \textbf{learning rate}, that scales the size of each step.
    
    Because deep learning architectures involve the composition of layers, the derivative must be computed with the chain rule. An efficient algorithm for doing this is the \textbf{backpropogation} algorithm, where derivatives are pushed from the end to the start of the network. % REF APPENDIX 
\end{itemize}

 



%Cost of overfitting (need for regularization). - CAN BE ADDRESSED WITHIN DL

\textbf{Challenges:} 
% Necessity for Geometric approaches for reducing curse of dimensionality (WHICH CANNOT BE ADDRESSED WITHOUT CONSIDERED GEOMETRIC DL)
Usually, the more interesting the type of data, the higher dimension space it lives in.  For example, a small 64x64 image is an element of $\mathcal{R}^{12288}$. In such situations, models experience a class of phenomena called ``curse of dimensionality''. I describe some of these below and point to \cite{altman2018curse} for a more thorough elaboration:
\begin{itemize}
    \item \textbf{Combinatorial Blow Up}: Consider sampling from $\{0,1\}^n$. The number of possible samples grows with $O(2^n)$, demanding an exponential increase in the number of samples required to cover the same proportion of space.
    \item \textbf{Data Sparsity}: Increasing the dimensionality of the space increases its volume. Points also get further away from each other because there are more components to contribute positively to distance. Lastly, the probability a point is not anomalous in any dimension becomes vanishingly small even with a tiny probability of deviating from the mean. All these contribute to the data being sparse. This means that new observations will be significantly dissimilar from old observations.
\end{itemize}

\subsection{Geometric Deep Learning}
\label{sec:gdl}
This \cite{bronstein2021geometric} unifying perspective on deep learning proposes to solve the curse of dimensionality by exploiting certain geometric symmetries. By baking such inductive biases into the architecture, it becomes easier for the model to reinterpret the high dimensional input as intrinsically low dimension. I now present two architecture families that make use of these geometric priors.

Note, it is also possible to encode geometric priors by using suitable data augmentation techniques, although this is less efficient.

\subsection{Convolutional Neural Network}
\label{sec:CNN}

%TODO spend more time explaining clearly what a filter is and how it relates to convolutions

The \textbf{Convolutional Neural Networks} (CNN) defines a class of architectures for operating over grid-like topologies, such as images. They exploit the prior that the data should be \textbf{shift equivarient}; that is, translating the input leads to an equal translation in the output, or $f(t(x)) = t(f(x))$ where $f$ is the function and $t$ is the translation. 

%\footnote{Technically, the CNN encodes a shift \textbf{equivariance} prior}
There are two defining qualities of the CNN: its use of \textbf{convolutions} and \textbf{downsampling}. I present them below, and then follow by mentioning a particularly noteworthy architecture, the ResNet.

\subsubsection{Convolutions}
\label{sec:convolutions}
Mathematically, a convolution is a binary operator $*:(F\times F)\rightarrow F$ that takes a pair of functions $f$ \& $g$ and returns another $f*g$ where:

$$(f*g)(t) \triangleq \int_{-\infty}^{\infty}f(x)\times g(t-x) dx$$

At each value of t, $g$ is reversed and shifted by that amount. It is then multiplied pointwise with $f$ and finally a sum is taken. It can be shown that convolving is commutative. In addition, convolution is \textbf{shift equivarient}. Consider an input signal denoted by $f$ that is convolved with ``kernel'' $g$:

\begin{equation}
    T_s(f*g)(t) = (T_s(f)*g)(t)
    \label{eq:shift_eq}
\end{equation}

where $T_s(f)(t) \triangleq f(t+s)$. In otherwords, shifting then convolving gives the same result as convolving then shifting, exactly what is needed for shift equivariance.

The convolutional layer, popularised by LeCun \cite{lecun1998gradient}, is a discrete (and often two dimensional) instance of a convolution. The input signal $f$ is replaced with pixels of an image, and the kernel $g$ is replaced with a ``filter'', a small matrix of learnable weights. Naturally, convolving the image with the filter involves placing the filter on each patch of the image, multipying pairwise, then summing. The same filter is moved across the input so that it overlaps on top of different receptive fields, with the output across the whole image being referred to as a \textbf{feature map}. A single convolutional layer will usually contain several filters that operate in parallel and which produce a collection of feature maps.

    \begin{figure}[H]
        \centering
        \includegraphics[width=14cm,height=6cm,keepaspectratio]{Resources/cnn filter.png}
        \caption{A convolutional filter being applied. Taken from \cite{cnn_image_ref}}
        \label{fig:conv}
    \end{figure}

Pre-defined filters have their own place within computer vision. Prewitt and Sobel filters are used for edge detection, and the Gaussian Blur filter is used for smoothing.
%TODO CITE

\begin{figure}[H]
    \centering
    \subfloat[\centering]{$ \begin{bmatrix}
+1 & 0 & -1 \\
+1 & 0 & -1 \\
+1 & 0 & -1 
\end{bmatrix}  $}%
    \qquad
    \subfloat[\centering]{$ \begin{bmatrix}
+1 & 0 & -1 \\
+2 & 0 & -2 \\
+1 & 0 & -1 
\end{bmatrix}  $}%
    \caption{The Horizontal Prewitt Filter (a), The Horizontal Sobel Filter (b)}%
    \label{fig:hovernet_importance}%
\end{figure}


Images are composed of a hierarchy of visual objects. The earlier convolutional layer learns to recognise the most basic of features, edges and corners, which the later layers can use to construct more complex objects, like circles, eyes and heads. The layers work their way up the hierarchy until something as visually rich as a person can be recognised. 

\subsubsection{Downsampling}
Each convolution provides information about neighbours to each cell in the grid. It is through this ``message-passing'' that cells can update their beliefs of the entire space. One option to connect distant cells is to use a larger kernel. Unfortunately, increasing the kernel size comes at a steep computational cost, not to mention the increase in training examples required to compensate for the rise in parameters. 

A solution is to use \textbf{pooling}, where blocks of adjacent cells are reduced to a single cell, thus shortening distances. Examples include \textbf{average pooling} and \textbf{max pooling}, where the mean and maximum of a block (say 2x2) is taken to be the representative.

Downsampling can also be achieved by modifying the \textbf{stride} of convolutions. The stride denotes the step size when moving the filter across feature maps. A stride of 2 will anchor on ever other pixel, and will yield a grid with similar dimensions to a 2x2 max pool.

\subsubsection{ResNet}
The main contribution of the Residual Network (ResNet) \cite{resnet} is to place skip connections between blocks of convolutions. 

It is hard to know in advance how many layers are required to properly process an input. Because each layer approximately mimics the zero function by default, adding an untrained extra layer to an existing model will cause predictions to fail. Skip connections solve this problem by making (blocks of) layers default to the identity function. They do this by adding the output of layers (the residual) to the input; by default the residual is near zero.

\begin{figure}[H]
    \centering
    \includegraphics[width=6cm,height=6cm,keepaspectratio]{Resources/skip_connection.PNG}
    \caption{A skip connection from the original paper \cite{resnet}}%
    \label{fig:res_connection}%
\end{figure}



% Altenating between conv, relu, batch and pool
% need for residual connections
% fully connected layers at end

% Different sizes and specifications

\subsection{Graph Neural Network}
\label{sec:GNN_intro}
%TODO CITE PETAR
When moving from grids to graphs, we gain and lose certain geometric priors; for example, graphs have no concept of position or orientation, so we can ignore shift equivariance. Graphs remain isomorphic under relabelling of nodes, and operations acting over graphs must respect this. This requirement is captured by \textbf{permutation} priors. 

%TODO

A weighted graph is mathematically defined with a pair $G=(V,E)$, where $V$ is the set of nodes ($|V|=n$) and $E$ the set of weighted edges. Concrete definitions will encapsulate both of these into an adjacency matrix $A \in \mathcal{R}^{n \times n}$ which stores weights between all pairs of nodes. In addition, we may choose to store information about each node - called a \textbf{node embedding} - with a vector $v \in \mathcal{R}^m$; these vectors are then stacked to create a ``feature matrix'' $X \in \mathcal{R}^{n\times m}$. If we relabel nodes, the feature and adjacency matrix would be permuted accordingly, namely $X \mapsto PX$ \& $A \mapsto PAP^T$ where $P$ is the corresponding permutation matrix.

\begin{equation}
    f(PX,PAP^T) = f(X,A)
    \tag{Perm. Invariance}
\end{equation}

\begin{equation}
    f(PX,PAP^T) = Pf(X,A)
    \tag{Perm. Equivariance}
\end{equation}


The above equations define what it means for a function to adhere to these priors. Functions computing global properties of graphs (such as graph classifiers) should ideally be \textbf{permutation invariant}, while functions that compute or transform nodes should be \textbf{permutation equivariant}.

As with CNNs, the key building blocks of \textbf{Graph Neural Networks} are its convolution and pooling layers.

\subsubsection{Graph Convolutions}
\label{sec:graph_convolution}
Recall that image convolutions act on local receptive fields. Information from adjacent pixels is aggregated by multiplying them by some learned weight, and then summing.

Graph convolutions followed a similar pattern:
\begin{itemize}
    \item \textbf{Receptive Field}: The receptive field of a node $x_i$ in a graph are its neighbours $N(x_i)$.
    \item \textbf{Message Passing}: Each node receives information about its neighbour in the form of a message. Messages are some function of both the sender and receiver. A message from node $i$ to $j$ is denoted by $\psi(x_i,x_j)$.
    \item \textbf{Aggregation}: The set of messages are aggregated or reduced to a single vector, using an operator like sum, mean or max, generally denoted with $\oplus$.
\end{itemize}

Message passing and aggregation are respectively equivariant and invariant under permutation, making them appealing candidates for processing graphs. The final step is to take our node $x_i$ with the aggregation of its neighbours' messages and generate a new embedding $h_i$. This is summarised below \cite{bronstein2021geometric}:

$$h_i = \phi\left( x_i,\bigoplus_{x_j\in N(x_i)} \psi(x_i,x_j)\right)$$

\begin{figure}[H]
        \centering
        \includegraphics[width=6cm,height=6cm,keepaspectratio]{Resources/mpnn.png}
        \caption{General Message Passing Convolution on a Receptive Field. Taken from \cite{bronstein2021geometric}}
        \label{fig:mpnn}
    \end{figure}
In the literature, three flavours of GNN convolutions are usually presented: \textbf{convolutional}, \textbf{attentional}, \textbf{message passing}. These are in fact all examples of message passing with increasing laxness on the form of $\psi(x_i,x_j)$; it is for this reason that I have only presented the most general form.



\subsubsection{Pooling}
Pooling comes in two main flavours: local and global. Local or hierarchical pooling aims to achieve the same goals as downsampling in a CNN, namely to reduce the size of the data while preserving information; this is so messages can travel shorter distances to reach far away nodes. In images, downsampling reduced blocks of pixels to a single point, while in graphs, it is typically clusters that are reduced to a representative node.

\begin{figure}[H]
        \centering
        \includegraphics[width=10cm,height=6cm,keepaspectratio]{Resources/hierarchical_pooling.PNG}
        \caption{Hierarchical Pooling from \cite{ying2018hierarchical}}
        \label{fig:hierarchical_pooling}
    \end{figure}

When it comes to classifying an entire graph - which will be the objective of my GNN model - the approach must be able to handle any sized graph, both very large and very small. Global pooling can be used to reduce any graph to a fixed sized vector by performing an aggregation across all node embeddings. This final vector encodes a meaningful summary of the graph, and an MLP network can be trained to predict classes from it. Popular global pooling layers include \textbf{global average pooling} and \textbf{global max pooling}.
\section{Explainable AI}

The goals of Explainable AI (XAI) are four fold \cite{adadi2018peeking}: 1) To justify model's decisions, 2) To control and check for erroneous behaviour, 3) To help test and improve the model, 4) To provide insights and new discovers relating to the task. It is the shroud of model complexity that makes task one non-trivial, effectively turning the model into an opaque ``black-box''.  Below, I justify the value of model complexity and then discuss techniques for alleviating its shortcomings.
% Interpretability vs Explainability

Tasks in machine learning can often be reformulated as curve-fitting problems. A parameterised model implicitly defines a set of ``curves'' that it can represent. For example, linear models capture all possible straight lines. There will be an unavoidable error if the true curve is not an element of the set of functions \footnote{\cite{bottou2007tradeoffs} gives a decomposition of a model's error}. A \textbf{universal approximator} is a model that defines a dense set of curves and thus sends this error to zero. \cite{hornik1989multilayer} shows that the MLP is an example of a universal approximator. 

The weakness of MLPs versus linear models is their lack of \textbf{interpretability}, which \cite{miller2017explanation} defines as ``the degree to which
an observer can understand the cause of a decision''. \cite{johansson2011trade} points towards a fundamental trade-off between accuracy and interpretability.

\begin{figure}[H]
        \centering
        \includegraphics[width=10cm,height=4cm,keepaspectratio]{Resources/inter_vs_acc.PNG}
        \caption{Different ML models on a notional accuracy vs interpretability graph, taken from \cite{morocho2019machine}}
        \label{fig:inter_vs_acc_fig}
    \end{figure}
    

%  Importance (problems of counter factual) vs Concept based (higher level units are more interpretable)
Explainability mechanisms can be used to make models more transparent and interpretable. I briefly present two example approaches:
\begin{itemize}
    \item \textbf{Attribution Methods} \cite{ancona2017towards}: Layer-wise Relevance Propogation \cite{binder2016layer} and DeepLIFT \cite{shrikumar2017learning} attempt to quantify the contribution of the inputs to the outputs by making use of the corresponding derivatives. This aims to reflect the importance the model places on certain features of the input and is typically visualised in a heatmap. % PROBLEM OF COUNTER FACTUALS % PROBLEM OF LOCALTY.
    \item \textbf{Concept-based Methods}: A concept is a high-level unit of information that plays a significant role in the decision making process. For images, these manifest as ``superpixels'' \cite{achantaSLICSuperpixelsCompared2012} formed by clustering adjacent and similar pixels together. \cite{koh2020concept} discusses \textbf{concept bottleneck} models where the network (in the form $f(g(x))$) is forced to learn concepts (with an encoder $g$) before using them to make a prediction (with a classifier $f$). If $f$ is easily interpretable, then explanations can be understood in terms of the concepts present in the data. This approach also lends itself to ``human-in-the-loop'' setups where users can amend incorrectly detected concepts in order to update predictions. Concepts can either be generated in a supervised manner, where labels exist for each of the predefined concepts, or in an unsupervised manner, where they are discovered \cite{ghorbani2019towards}.
\end{itemize}


This project will examine an explainability framework called \textbf{GCExplainer} \cite{magister2021gcexplainer} which explains GNN predictions with the use of automatically discovered concepts.
%Linear in terms of higher level concepts
% Concept based with linear is good idea

% Different explainability models for different 


\section{Software Engineering} %KEEP CONCISE
\subsection{Requirements Analysis}
Below are the five stages of my pipeline that I proposed to implement:
\begin{enumerate}
    \item \textbf{Stain Normalisation}: Implement an algorithm for normalising H\&E stains.
    \item \textbf{Nuclear Panoptic Segmentation}: Implement a deep learning model for identifying and classifying nuclei.
    \item \textbf{Cell Graph Construction}: Define and create a cell graph.
    \item \textbf{Cell Graph Classification}: Implement a graph neural network to classify the presence of cancer in graph from (3).
    \item \textbf{GCExplainer}: Implement a post-hoc explainability algorithm, namely GCExplainer, to make the model in (4) more interpretable.
\end{enumerate}

These requirements differ to the proposal only in their specificity: Steps 1-3 correspond to step 1 in the proposal, steps 4 \& 5 to steps 2 \& 3 respectively.

\subsection{Language and Libraries}
I completed this project in \textbf{Python} with the use of, but not limited to, the following libraries:
%Language
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[H]
\begin{tabular}{lll}
\hline
\textbf{Library} & \textbf{Purpose}                   & \textbf{License}   \\ \hline
numpy            & Data manipulation library          & BSD license        \\
scipy             & \begin{tabular}[c]{@{}l@{}}Scientific computing library, with optimization \\ and image algorithms\end{tabular} & BSD license \\
mlflow           & An ML experiment logger            & Apache license 2.0 \\
Pytorch          & Deep Learning framework            & BSD license        \\
Pytorch Geometric & Extension of Pytorch to operate over graphs                                                                     & MIT license \\
matplotlib       & Plotting and visualization library & PSF license        \\
opencv-python    & Image processing library           & Apache license 2.0 \\
networkx         & Creating and manipulating graphs   & BSD license       
\end{tabular}
\end{table}

I chose Python because of both my familiarity with the language and the aforementioned library support. I worked in \texttt{Visual Studio Code} and used \texttt{Jupyter Notebooks} to record my steps. In addition, I used \textbf{Pytorch Lightning} to structure my architectures and training; it is considered by some to be a standard for submitting deep learning code a conferences, which is why I opted to use it. 

\subsubsection{Starting Point}
Prior to this project, I had studied the basics of deep learning in my own time and worked with \textbf{numpy}, \textbf{scipy}, \textbf{Pytorch} and \textbf{matplotlib}. However, I did not have experience with GNNs, segmentation algorithms, image processing algorithms and libraries like \textbf{opencv}, explainable AI, or an understanding of the biological prerequisites discussed.

Best-practises with handling data and conducting experiments learned from the Part II ``Advanced Data Science'' and ``Machine Learning \& Bayesian Inference" courses proved to be invaluable.


\subsection{Working Environment}
\subsubsection{Hardware}
Heavy workloads were run on my desktop's \texttt{NVIDIA GeForce 1080 GTX}, which houses 8GB of GPU memory. I worked remotely on my laptop and connected to my desktop through SSH \& a VPN.

\subsubsection{Backups and Testing}
Backups were not only important for managing the project's risk but also for supporting remote work: The code was \textbf{git} version controlled in a \textbf{GitHub} repository; The dissertation, written in overleaf, was routinely downloaded and saved on my personal \textbf{Google Drive}; A copy of the datasets (\textbf{PanNuke}\cite{gamperPanNukeDatasetExtension2020} and \textbf{BACH}\cite{aresta2019bach}) was stored in a \textbf{Google Cloud} storage bucket.

In addition, I wrote some python unit tests in \textbf{pytest}. Due to the probabilistic nature of most of the algorithms and the sequential dependencies between the steps, it was hard to define concrete test cases for anything other than the data preparation and processing steps. Regardless, the code was vetted with constant visualisation of outputs and assertion statements throughout.
% GIT
% Google Drive
% Data saved on Google Cloud Platform bucket with a script

